Information dynamics and symmetry breaking in generic monitored $\mathbb{Z}_2$-symmetric open quantum systems

We investigate the steady-state phases of generic $\mathbb{Z}_2$-symmetric monitored, open quantum dynamics. We describe the phases systematically in terms of both information-theoretic diagnostics and spontaneous breaking of strong and weak symmetries of the dynamics. We find a completely broken phase where information is retained by the quantum system, a strong-to-weak broken phase where information is leaked to the environment, and an unbroken phase where information is learned by the observer. We find that weak measurement and dephasing alone constitute a minimal model for generic open systems with $\mathbb{Z}_2$ symmetry, but we also explore perturbations by unitary gates. For a 1d set of qubits, we examine information-theoretic and symmetry-breaking observables in the path integral of the doubled state. This path integral reduces to the standard classical 2d random-bond Ising model in certain limits but generically involves negative weights, enabling a special self-dual random-bond Ising model at the critical point when only measurements are present. We obtain numerical evidence for the steady-state phases using efficient tensor network simulations of the doubled state.

==> x_meas_simple.tex <==
\begin{scope}[line join=round]

  % Offset for the back square
  \def\dx{0.3}
  \def\dy{0.3}

  % Back square (lighter red), shifted up-right
  \begin{scope}[shift={(\dx,\dy)}]
    \filldraw[red!30, draw=black, thick] (0,0) rectangle (1,1);
  \end{scope}

  % Front square (darker red)
  \filldraw[red!60, draw=black, thick] (0,0) rectangle (1,1);

  % Short top circuit line from front square
  \draw[thick] (0.5,1) -- ++(0,\dy);

  % Center label
  \node at (0.5,0.5) {\large \( X \)};

\end{scope}

==> x_noise_simple.tex <==
\begin{scope}[line join=round, line cap=round]

  \def\dx{0.3}
  \def\dy{0.3}

  % Front face corners
  \coordinate (FBL) at (0,0);
  \coordinate (FBR) at (1,0);
  \coordinate (FTL) at (0,1);
  \coordinate (FTR) at (1,1);

  % Back face corners
  \coordinate (BBL) at ($(FBL)+(\dx,\dy)$);
  \coordinate (BBR) at ($(FBR)+(\dx,\dy)$);
  \coordinate (BTL) at ($(FTL)+(\dx,\dy)$);
  \coordinate (BTR) at ($(FTR)+(\dx,\dy)$);

  % Back face border first
  \draw[thick] (BBL) -- (BBR) -- (BTR) -- (BTL) -- cycle;

  % Fill faces
  \fill[yellow!50] (BBL) -- (BBR) -- (BTR) -- (BTL) -- cycle;
  \fill[yellow!70] (BBL) -- (BTL) -- (FTL) -- (FBL) -- cycle;
  \fill[yellow!40] (BBR) -- (FBR) -- (FTR) -- (BTR) -- cycle;
  \fill[yellow!60] (BTL) -- (BTR) -- (FTR) -- (FTL) -- cycle;
  \fill[yellow]    (FBL) -- (FBR) -- (FTR) -- (FTL) -- cycle;

  % Stroke front-facing edges
  \draw[thick] (FBL) -- (FBR) -- (FTR) -- (FTL) -- cycle;
  \draw[thick] (FBR) -- (BBR);
  \draw[thick] (FTL) -- (BTL);
  \draw[thick] (FTR) -- (BTR);
  \draw[thick] (BTL) -- (BTR);
  \draw[thick] (BTR) -- (BBR);

  % Short top circuit line
  \draw[thick] ($(FTL)!0.5!(FTR)$) -- ++(0,\dy);

  % Label
  \node at ($(FBL)!0.5!(FTR)$) {\large \( X \)};

\end{scope}


==> zz_meas_simple.tex <==
\begin{scope}[line join=round]

  \def\dx{0.3}
  \def\dy{0.3}

  % Back square (lighter blue), shifted up-right
  \begin{scope}[shift={(\dx,\dy)}]
    \filldraw[blue!30, draw=black, thick] (0,0) rectangle (1,1);
  \end{scope}

  % Front square (darker blue)
  \filldraw[blue!60, draw=black, thick] (0,0) rectangle (1,1);

  % Short vertical circuit lines from left and right top corners
  \draw[thick] (0,1) -- ++(0,\dy);
  \draw[thick] (1,1) -- ++(0,\dy);

  % Gate label
  \node at (0.5,0.5) {\large \( ZZ \)};

\end{scope}


==> zz_noise_simple.tex <==
\begin{scope}[line join=round, line cap=round]

  \def\dx{0.3}
  \def\dy{0.3}

  % Front face
  \coordinate (FBL) at (0,0);
  \coordinate (FBR) at (1,0);
  \coordinate (FTL) at (0,1);
  \coordinate (FTR) at (1,1);

  % Back face
  \coordinate (BBL) at ($(FBL)+(\dx,\dy)$);
  \coordinate (BBR) at ($(FBR)+(\dx,\dy)$);
  \coordinate (BTL) at ($(FTL)+(\dx,\dy)$);
  \coordinate (BTR) at ($(FTR)+(\dx,\dy)$);

  % Back face border
  \draw[thick] (BBL) -- (BBR) -- (BTR) -- (BTL) -- cycle;

  % Fill faces
  \fill[yellow!50] (BBL) -- (BBR) -- (BTR) -- (BTL) -- cycle;
  \fill[yellow!70] (BBL) -- (BTL) -- (FTL) -- (FBL) -- cycle;
  \fill[yellow!40] (BBR) -- (FBR) -- (FTR) -- (BTR) -- cycle;
  \fill[yellow!60] (BTL) -- (BTR) -- (FTR) -- (FTL) -- cycle;
  \fill[yellow]    (FBL) -- (FBR) -- (FTR) -- (FTL) -- cycle;

  % Edges
  \draw[thick] (FBL) -- (FBR) -- (FTR) -- (FTL) -- cycle;
  \draw[thick] (FBR) -- (BBR);
  \draw[thick] (FTL) -- (BTL);
  \draw[thick] (FTR) -- (BTR);
  \draw[thick] (BTL) -- (BTR);
  \draw[thick] (BTR) -- (BBR);

  % Short circuit lines from top front corners
  \draw[thick] (FTL) -- ++(0,\dy);
  \draw[thick] (FTR) -- ++(0,\dy);

  % Label
  \node at ($(FBL)!0.5!(FTR)$) {\large \( ZZ \)};

\end{scope}

